An Existence Theorem of Nash Equilibrium in Coq and Isabelle

Nash equilibrium (NE) is a central concept in game theory. Here we prove formally a published theorem on existence of an NE in two proof assistants, Coq and Isabelle: starting from a game with finitely many outcomes, one may derive a game by rewriting each of these outcomes with either of two basic outcomes, namely that Player 1 wins or that Player 2 wins. If all ways of deriving such a win/lose game lead to a game where one player has a winning strategy, the original game also has a Nash equilibrium. This article makes three other contributions: first, while the original proof invoked linear extension of strict partial orders, here we avoid it by generalizing the relevant definition. Second, we notice that the theorem also implies the existence of a secure equilibrium, a stronger version of NE that was introduced for model checking. Third, we also notice that the constructive proof of the theorem computes secure equilibria for non-zero-sum priority games (generalizing parity games) in quasi-polynomial time.

==> eptcsdata.tex <==
\providecommand{\firstpage}{46}
\providecommand{\publicationstatus}{P. Bouyer, A. Orlandini \& P. San Pietro (Eds.): 8th Symposium on\\ Games, Automata, Logics and Formal Verification (GandALF'17)\\
EPTCS 256, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.256.4}{10.4204/EPTCS.256.4}}
\pdfoutput=1

